Generalization by design: Shortcuts to Generalization in Deep Learning

We take a geometrical viewpoint and present a unifying view on supervised deep learning with the Bregman divergence loss function - this entails frequent classification and prediction tasks. Motivated by simulations we suggest that there is principally no implicit bias of vanilla stochastic gradient descent training of deep models towards "simpler" functions. Instead, we show that good generalization may be instigated by bounded spectral products over layers leading to a novel geometric regularizer. It is revealed that in deep enough models such a regularizer enables both, extreme accuracy and generalization, to be reached. We associate popular regularization techniques like weight decay, drop out, batch normalization, and early stopping with this perspective. Backed up by theory we further demonstrate that "generalization by design" is practically possible and that good generalization may be encoded into the structure of the network. We design two such easy-to-use structural regularizers that insert an additional \textit{generalization layer} into a model architecture, one with a skip connection and another one with drop-out. We verify our theoretical results in experiments on various feedforward and convolutional architectures, including ResNets, and datasets (MNIST, CIFAR10, synthetic data). We believe this work opens up new avenues of research towards better generalizing architectures.

==> 01motivation.tex <==
\section{Motivation}
\section{Sidenotes on the learning rate effects}
\subsection{GD with fixed learning rate escapes narrow valleys naturaly}

Often there is a notion of SGD, opposed to full GD, to be prone to escape local minima of loss function because of the stochastic dynamics induced by the gradient noise \cite{du2018gradient, li2017stochastic, li2018visualizing, lange1995gradient} \todo{check refs and add more}. It is also known that learning rate is one of the most important hyperparameters in terms of convergence.

In the following we motivate a notion of fixed learning rate being important not only in terms of convergence but also in respect of generalization. In particular we take an intuitive and widely accepted property of fixed (inaccurate) learning rate avoids optima that are too narrow with respect to learning rate and drive GD and SGD into shallow valleys analyze it and draw conclusions.

To showcase the behaviour we take cosine with a phase dependent on $4th$ power of Euclidean distance from an origin. That is an extremely nonconvex loss function with high barriers between optima as follows: 
\begin{align}
    &-\cos{\{x^4\pi\//c^4}\} \tag{1D cosine loss} \label{def:1dcos_los} \\
    &-\cos{\{(x+y)^4\pi\//c^4}\} \tag{2D cosine loss} \label{def:2dcos_los}
\end{align}
where $c$ is chosen fixed constant ($c:=1\//15$ in our experiments) and run both gradient descent and stochastic gradient descent with a fixed learning rate $\eta$ in order to find the optima. For \ref{def:1dcos_los} all local optima are given by a set $\hat{x} \in \{c\sqrt[4]{n}, n \in \mathrm{N}^{+}\}$ which for $c:=15$, chosen for experiments in Fig.\ref{fig:toy_experiments_cosine_1D} and Fig.\ref{fig:toy_experiments_cosine_2D}, gives $\approx \{0,15,17.84,19.74,21.21, \dots \}$ with a span between the first two local \textit{minima} being $\approx \{17.84,3.57\}$ and further diminishing as $|x| \xrightarrow{} \infty$. As a density of stationary points grows over all limits with $|x| \xrightarrow{} \infty$ we'd like to study convergence of a (stochastic) gradient descent initialized in the highly rugged region.

Results of gradient descent and stochastic variant of the same for both losses are presented in Fig. \eqref{fig:toy_experiments_cosine_1D} and \eqref{fig:toy_experiments_cosine_2D}. Experiments demonstrate \todo{\dots} not suprisingly we observe that narrow both GD and SGD are converge toward flat minima ina sea
\begin{figure*}[h!]
    \centering
\begin{subfigure}[t]{.3\linewidth}
\centering
  \includegraphics[width=.95\linewidth]{img/gd1D_eta0_5.png}
   \caption{}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
    \includegraphics[width=.95\linewidth]{img/gd1D_eta1_5.png}
    \caption{}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
    \includegraphics[width=.95\linewidth]{img/gd1D_eta20.png}
    \caption{}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
  \includegraphics[width=.95\linewidth]{img/sgd1D_eta0_5.png}
   \caption{}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
    \includegraphics[width=.95\linewidth]{img/sgd1D_eta1_5.png}
    \caption{}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
    \includegraphics[width=.95\linewidth]{img/sgd1D_eta20.png}
    \caption{}
\end{subfigure}

\caption{\textbf{1D trajectory of GD (the first row) and SGD (the second row) over 300 steps}. The first row of the panel presents a trajectory of GD for different learning rates: $\eta \in \{0.5,1.5,2\}$ reported in (a), (b) and (c) respectively. The SGD is modeled in the second row where additive Gaussian noise of zero mean and $\sigma=0.5$ is added to gradients. Figures (d), (e), and (f) correspond to same learning rates as row above, i.e., $\eta \in \{0.5,1.5,2\}$ respectively. An initialization point $[40]$ is evacuated immediately and GD in the first row as well as SGD in the second row of the panel converges towards flatter regions, in spite of multiple optima and rugged landscape, until it settles in wide enough surroundings that produces gradients not large enough to overweight regularizing term $\norm{\bm{w}-\bm{w}_0}^2_2$ in Eq. \eqref{def:sgd_as_min}.}
\label{fig:toy_experiments_cosine_1D}
\end{figure*}

\begin{figure*}[h!]
    \centering
\begin{subfigure}[t]{.3\linewidth}
\centering
  \includegraphics[width=.95\linewidth]{img/cosine2D/gd2D_eta0.5.png}
   \caption{}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
    \includegraphics[width=.95\linewidth]{img/cosine2D/gd2D_eta15.0.png}
    \caption{}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
    \includegraphics[width=.95\linewidth]{img/cosine2D/gd2D_eta20.0.png}
    \caption{}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
  \includegraphics[width=.95\linewidth]{img/cosine2D/sgd2D_eta5.0.png}
   \caption{}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
    \includegraphics[width=.95\linewidth]{img/cosine2D/sgd2D_eta15.0.png}
    \caption{}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
    \includegraphics[width=.95\linewidth]{img/cosine2D/sgd2D_eta20.0.png}
    \caption{}
\end{subfigure}

\caption{\textbf{2D trajectory of GD (first row) and SGD (second row) over 300 steps}. In complete analogy to 1D experiment of Fig \eqref{fig:toy_experiments_cosine_1D} the first row of the panel presents trajecotyr of GD for different learning rates: $\eta \in \{0.5,1.5,2\}$ reported in (a), (b) and (c) respectively. The SGD is modeled in the second row where additive Gaussian noise of zero mean and $\sigma=0.5$ is added to gradients. Figures (d), (e), and (f) correspond to same learning rates as row above, i.e., $\eta \in \{0.5,1.5,2\}$ respectively. We again see that an initialization point $[-20,-20]$ is evacuated immediately and GD in the first row as well as SGD in the second row of the panel converges towards flatter regions, in spite of multiple optima and rugged landscape, until it settles in wide enough surroundings that produces gradients not large enough to overweight regularizing term $\norm{\bm{w}-\bm{w}_0}^2_2$ in Eq. \eqref{def:sgd_as_min}.}
\label{fig:toy_experiments_cosine_2D}
\end{figure*}

\subsubsection{weights and norms}

\begin{figure*}[h!]
    \centering
\begin{subfigure}[t]{.3\linewidth}
\centering
  \includegraphics[width=.95\linewidth]{img/momentum/histogram_mnist_cnn_epoch_1_lr0.01_b64_wnorms_random_with_momentum_gamma095_with_bias.png}
   \caption{}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
  \includegraphics[width=.95\linewidth]{img/momentum/histogram_mnist_cnn_epoch_100_lr0.01_b64_wnorms_wo_momentum_gamma09_with_bias.png}
   \caption{}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
  \includegraphics[width=.95\linewidth]{img/momentum/histogram_mnist_cnn_epoch_100_lr0.01_b64_wnorms_random_with_momentum_gamma095_with_bias.png}
   \caption{}
\end{subfigure}
\caption{\textbf{Histogram of weights after $100^{th}$ epoch when zero training error has been reached}. Figure (a) depicts weights distribution after standard (He) initialization, while Fig.(b) shows weights distribution after reaching 98.6 test accuracy and Fig.(c) reports same but in case of fitting random labels with momentum (0.95) as described in \cite{zhang2016understanding} (test accuracy corresponds to random choice. i.e. approx. 10\%). We can observe that (c) with random labels resulted in more complex model with significantly more weights being updated compared to initialization (a) than model fully convergent and well generalizing model (b). This suggests momentum accelerates training along the low curvature directions and allows SGD to reach far locations compared to no momentum, that did not converge whatsoever (not reported).}
\label{fig:momentum_experiments}
\end{figure*}

\subsubsection{momentum}

\begin{figure*}[h!]
    \centering
\begin{subfigure}[t]{.45\linewidth}
\centering
  \includegraphics[width=.95\linewidth]{img/momentum/train_errors_by_momentum_mnist_cnn_cranking_momentum0.01.png}
   \caption{}
\end{subfigure}
\begin{subfigure}[t]{.45\linewidth}
\centering
  \includegraphics[width=.95\linewidth]{img/momentum/train_errors_by_momentum_cifar10_cnncranking_momemntum0.01.png}
   \caption{}
\end{subfigure}
\caption{\textbf{Fitting random labels with momentum}. In complete analogy to \cite{zhang2016understanding} this figure reports training error ($y$ axis) of CNN classifying a) MNIST and (b) CIFAR10 \textbf{with random labels} with regards to momentum coefficient ($x$ axis). Notably on both datasets model is not able to learn random labels until momentum acceleration is used. Fig (a) suggests there is rather fast transition from non-convergent levels below 0.5 to convergent levles (in terms of training error) while Fig (b) on CIFAR10 shows similar but less rapid transition. We note that CIFAR10 model (b) runs 600 epochs to reach close to zero training error while MNIST (a) of 100 epochs. Working hypothesis being that this long training helped further by momentum enables SGD to get far from initialization to find complex overfitting solution of zero training error. But since training takes long even lower levels of momentum enhancement enables  SGD to converge. DISCLAIMER: Experiments still in progress -- to be continued}
\label{fig:weights_histograms}
\end{figure*}

==> notes_on_learning_rate_effects.tex <==
\section{Sidenotes on the learning rate effects}
\subsection{GD with fixed learning rate escapes narrow valleys naturaly}

Often there is a notion of SGD, opposed to full GD, to be prone to escape local minima of loss function because of the stochastic dynamics induced by the gradient noise \cite{du2018gradient, li2017stochastic, li2018visualizing, lange1995gradient} \todo{check refs and add more}. It is also known that learning rate is one of the most important hyperparameters in terms of convergence.

In the following we motivate a notion of fixed learning rate being important not only in terms of convergence but also in respect of generalization. In particular we take an intuitive and widely accepted property of fixed (inaccurate) learning rate avoids optima that are too narrow with respect to learning rate and drive GD and SGD into shallow valleys analyze it and draw conclusions.

To showcase the behaviour we take cosine with a phase dependent on $4th$ power of Euclidean distance from an origin. That is an extremely nonconvex loss function with high barriers between optima as follows: 
\begin{align}
    &-\cos{\{x^4\pi\//c^4}\} \tag{1D cosine loss} \label{def:1dcos_los} \\
    &-\cos{\{(x+y)^4\pi\//c^4}\} \tag{2D cosine loss} \label{def:2dcos_los}
\end{align}
where $c$ is chosen fixed constant ($c:=1\//15$ in our experiments) and run both gradient descent and stochastic gradient descent with a fixed learning rate $\eta$ in order to find the optima. For \ref{def:1dcos_los} all local optima are given by a set $\hat{x} \in \{c\sqrt[4]{n}, n \in \mathrm{N}^{+}\}$ which for $c:=15$, chosen for experiments in Fig.\ref{fig:toy_experiments_cosine_1D} and Fig.\ref{fig:toy_experiments_cosine_2D}, gives $\approx \{0,15,17.84,19.74,21.21, \dots \}$ with a span between the first two local \textit{minima} being $\approx \{17.84,3.57\}$ and further diminishing as $|x| \xrightarrow{} \infty$. As a density of stationary points grows over all limits with $|x| \xrightarrow{} \infty$ we'd like to study convergence of a (stochastic) gradient descent initialized in the highly rugged region.

Results of gradient descent and stochastic variant of the same for both losses are presented in Fig. \eqref{fig:toy_experiments_cosine_1D} and \eqref{fig:toy_experiments_cosine_2D}. Experiments demonstrate \todo{\dots} not suprisingly we observe that narrow both GD and SGD are converge toward flat minima ina sea
\begin{figure*}[h!]
    \centering
\begin{subfigure}[t]{.3\linewidth}
\centering
  \includegraphics[width=.95\linewidth]{img/gd1D_eta0_5.png}
   \caption{}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
    \includegraphics[width=.95\linewidth]{img/gd1D_eta1_5.png}
    \caption{}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
    \includegraphics[width=.95\linewidth]{img/gd1D_eta20.png}
    \caption{}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
  \includegraphics[width=.95\linewidth]{img/sgd1D_eta0_5.png}
   \caption{}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
    \includegraphics[width=.95\linewidth]{img/sgd1D_eta1_5.png}
    \caption{}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
    \includegraphics[width=.95\linewidth]{img/sgd1D_eta20.png}
    \caption{}
\end{subfigure}

\caption{\textbf{1D trajectory of GD (the first row) and SGD (the second row) over 300 steps}. The first row of the panel presents a trajectory of GD for different learning rates: $\eta \in \{0.5,1.5,2\}$ reported in (a), (b) and (c) respectively. The SGD is modeled in the second row where additive Gaussian noise of zero mean and $\sigma=0.5$ is added to gradients. Figures (d), (e), and (f) correspond to same learning rates as row above, i.e., $\eta \in \{0.5,1.5,2\}$ respectively. An initialization point $[40]$ is evacuated immediately and GD in the first row as well as SGD in the second row of the panel converges towards flatter regions, in spite of multiple optima and rugged landscape, until it settles in wide enough surroundings that produces gradients not large enough to overweight regularizing term $\norm{\bm{w}-\bm{w}_0}^2_2$ in Eq. \eqref{def:sgd_as_min}.}
\label{fig:toy_experiments_cosine_1D}
\end{figure*}

\begin{figure*}[h!]
    \centering
\begin{subfigure}[t]{.3\linewidth}
\centering
  \includegraphics[width=.95\linewidth]{img/cosine2D/gd2D_eta0.5.png}
   \caption{}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
    \includegraphics[width=.95\linewidth]{img/cosine2D/gd2D_eta15.0.png}
    \caption{}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
    \includegraphics[width=.95\linewidth]{img/cosine2D/gd2D_eta20.0.png}
    \caption{}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
  \includegraphics[width=.95\linewidth]{img/cosine2D/sgd2D_eta5.0.png}
   \caption{}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
    \includegraphics[width=.95\linewidth]{img/cosine2D/sgd2D_eta15.0.png}
    \caption{}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
    \includegraphics[width=.95\linewidth]{img/cosine2D/sgd2D_eta20.0.png}
    \caption{}
\end{subfigure}

\caption{\textbf{2D trajectory of GD (first row) and SGD (second row) over 300 steps}. In complete analogy to 1D experiment of Fig \eqref{fig:toy_experiments_cosine_1D} the first row of the panel presents trajecotyr of GD for different learning rates: $\eta \in \{0.5,1.5,2\}$ reported in (a), (b) and (c) respectively. The SGD is modeled in the second row where additive Gaussian noise of zero mean and $\sigma=0.5$ is added to gradients. Figures (d), (e), and (f) correspond to same learning rates as row above, i.e., $\eta \in \{0.5,1.5,2\}$ respectively. We again see that an initialization point $[-20,-20]$ is evacuated immediately and GD in the first row as well as SGD in the second row of the panel converges towards flatter regions, in spite of multiple optima and rugged landscape, until it settles in wide enough surroundings that produces gradients not large enough to overweight regularizing term $\norm{\bm{w}-\bm{w}_0}^2_2$ in Eq. \eqref{def:sgd_as_min}.}
\label{fig:toy_experiments_cosine_2D}
\end{figure*}

\subsubsection{weights and norms}

\begin{figure*}[h!]
    \centering
\begin{subfigure}[t]{.3\linewidth}
\centering
  \includegraphics[width=.95\linewidth]{img/momentum/histogram_mnist_cnn_epoch_1_lr0.01_b64_wnorms_random_with_momentum_gamma095_with_bias.png}
   \caption{}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
  \includegraphics[width=.95\linewidth]{img/momentum/histogram_mnist_cnn_epoch_100_lr0.01_b64_wnorms_wo_momentum_gamma09_with_bias.png}
   \caption{}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
  \includegraphics[width=.95\linewidth]{img/momentum/histogram_mnist_cnn_epoch_100_lr0.01_b64_wnorms_random_with_momentum_gamma095_with_bias.png}
   \caption{}
\end{subfigure}
\caption{\textbf{Histogram of weights after $100^{th}$ epoch when zero training error has been reached}. Figure (a) depicts weights distribution after standard (He) initialization, while Fig.(b) shows weights distribution after reaching 98.6 test accuracy and Fig.(c) reports same but in case of fitting random labels with momentum (0.95) as described in \cite{zhang2016understanding} (test accuracy corresponds to random choice. i.e. approx. 10\%). We can observe that (c) with random labels resulted in more complex model with significantly more weights being updated compared to initialization (a) than model fully convergent and well generalizing model (b). This suggests momentum accelerates training along the low curvature directions and allows SGD to reach far locations compared to no momentum, that did not converge whatsoever (not reported).}
\label{fig:momentum_experiments}
\end{figure*}

\subsubsection{momentum}

\begin{figure*}[h!]
    \centering
\begin{subfigure}[t]{.45\linewidth}
\centering
  \includegraphics[width=.95\linewidth]{img/momentum/train_errors_by_momentum_mnist_cnn_cranking_momentum0.01.png}
   \caption{}
\end{subfigure}
\begin{subfigure}[t]{.45\linewidth}
\centering
  \includegraphics[width=.95\linewidth]{img/momentum/train_errors_by_momentum_cifar10_cnncranking_momemntum0.01.png}
   \caption{}
\end{subfigure}
\caption{\textbf{Fitting random labels with momentum}. In complete analogy to \cite{zhang2016understanding} this figure reports training error ($y$ axis) of CNN classifying a) MNIST and (b) CIFAR10 \textbf{with random labels} with regards to momentum coefficient ($x$ axis). Notably on both datasets model is not able to learn random labels until momentum acceleration is used. Fig (a) suggests there is rather fast transition from non-convergent levels below 0.5 to convergent levles (in terms of training error) while Fig (b) on CIFAR10 shows similar but less rapid transition. We note that CIFAR10 model (b) runs 600 epochs to reach close to zero training error while MNIST (a) of 100 epochs. Working hypothesis being that this long training helped further by momentum enables SGD to get far from initialization to find complex overfitting solution of zero training error. But since training takes long even lower levels of momentum enhancement enables  SGD to converge. DISCLAIMER: Experiments still in progress -- to be continued}
\label{fig:weights_histograms}
\end{figure*}
